Fast Controllable Diffusion Models for Undersampled MRI Reconstruction

Supervised deep learning methods have shown promise in undersampled Magnetic Resonance Imaging (MRI) reconstruction, but their requirement for paired data limits their generalizability to the diverse MRI acquisition parameters. Recently, unsupervised controllable generative diffusion models have been applied to undersampled MRI reconstruction, without paired data or model retraining for different MRI acquisitions. However, diffusion models are generally slow in sampling and state-of-the-art acceleration techniques can lead to sub-optimal results when directly applied to the controllable generation process. This study introduces a new algorithm called Predictor-Projector-Noisor (PPN), which enhances and accelerates controllable generation of diffusion models for undersampled MRI reconstruction. Our results demonstrate that PPN produces high-fidelity MR images that conform to undersampled k-space measurements with significantly shorter reconstruction time than other controllable sampling methods. In addition, the unsupervised PPN accelerated diffusion models are adaptable to different MRI acquisition parameters, making them more practical for clinical use than supervised learning techniques.

==> sections/s2.method_old.tex <==
\section{method}


The generative approach for MRI undersampling reconstruction involves controlled (or conditional) generation of an MR image consistent with the 
k-space measurement. 
We first briefly review two diffusion models (DDPM and DDIM) for uncontrolled (or unconditional) generation of general images, then describe a controllable sampling method for the MRI undersampling reconstruction. 


\begin{figure*}[!t]
    \centering
	\includegraphics[width=120mm]{imgs/fig1.jpg}
	\caption{Illustration of one prediction step from using the original DDIM free generation (a) and the proposed PPN controlled generation (b). (c) shows the reverse image generation processes with and without k-space measurement guidance.
	\label{fig:onestep}}
\end{figure*}


\subsection{Diffusion Models}

Diffusion models are a class of deep generative neural networks that progressively reduce noise in many small steps from a random Gaussian noise until a realistic synthetic image is generated, which is ideally distributed according to the true data distribution of the training samples.

\subsubsection{DDPM} In Denoising Diffusion Probabilistic Models (DDPMs) \cite{ho2020denoising}, the reverse process 
$p_{\bftheta}(\bfx_{0:T})=p(\bfx_{T})\prod_{t=1}^{T}p_{\bftheta}(\bfx_{t-1} \mid \bfx_{t})$ 
transforms a Gaussian noise
$\bfx_{T} \sim \calN(\mathbf{0},\bfI)$ 
to data $\bfx_{0}$ using Gaussian transition kernels:
\begin{equation}
	p_{\bftheta}(\bfx_{t-1} \mid \bfx_{t})=\calN(\bfx_{t-1};\mathbf{\mu}_{\bftheta}(\bfx_{t},t),\mathbf{\Sigma}_{\bftheta}(\bfx_{t},t))
\end{equation}% need to find a relationship with \epsilon_\theta
The forward process 
$q(\bfx_{1:T} \mid \bfx_{0}) = \prod_{t=1}^{T} q(\bfx_{t} \mid \bfx_{t-1})$ 
is a fixed Markov Chain with Gaussian transition kernel
\begin{equation}
	q(\bfx_{t} \mid \bfx_{t-1})
	=
	\calN(\bfx_{t}; \sqrt{1-\beta_{t}} \bfx_{t-1}, \beta_{t} \bfI),
\end{equation}
where $\beta_{1:T}$ is a variance schedule.
Sampling $\bfx_{t}$ in the forward process can be done in closed form for any
time step $t$:
\begin{equation}
	q(\bfx_{t} \mid \bfx_{0})=\calN(\bfx_{t};\sqrt{\bar{\alpha}_{t}}\bfx_{0},(1-\bar{\alpha}_{t})\bfI)  \label{eq_ddpm2}
\end{equation}
where $\bar{\alpha}_{t}=\prod_{1}^{t}(1-\beta_{t})$. 
As $T$ increases, $\bar{\alpha}_{t}$ approaches 0 and $q(\bfx_{T} \mid \bfx_{0})$ reaches a standard normal distribution.
In addition, we can write 
\begin{equation}
	\bfx_{t} = \sqrt{\bar{\alpha}_{t}} \bfx_{0} + \sqrt{1 - \bar{\alpha}_{t}} \bm{\epsilon},
	\qquad \bm{\epsilon} \sim \calN(\mathbf{0},\bfI).
 \label{eq_fastforward}
\end{equation}

We can train the reverse process by first learning an noise prediction model
$\bm{\epsilon}_{\bftheta}(\bfx_{t}, t)$ via minimizing
$L(\bftheta) =\mathbf{E}_{t,\bfx_{0},\bm{\epsilon}}[\|\bm{\epsilon}-\bm{\epsilon}_{\bftheta}(\bfx_{t},t)\|^{2}]$, 
where $t$ is often uniformly distributed,
$\bfx_{0}$ follows the true data distribution $q(\bfx_{0})$, 
and $\bm{\epsilon} \sim \calN(\mathbf{0},\bfI)$. 
The reverse process is then defined as:
\begin{equation}
\bfx_{t-1}=\frac{1}{\sqrt{\alpha_{t}}}\left(\bfx_{t}-\frac{1-\alpha_{t}}{\sqrt{1-\bar{\alpha}_{t}}}\bm{\epsilon}_{\bftheta}(\bfx_{t},t)\right)+\sigma_{t}\mathbf{z} \label{eq_ddpm4}
\end{equation}
where $\mathbf{z}\sim\calN(\mathbf{0}$, 
$\bfI),\sigma_{t}=\sqrt{(1-\bar{\alpha}_{t-1})/(1-\bar{\alpha}_{t})}\cdot\sqrt{\beta_{t}}$.
The first term on the RHS is the expectation of   
$q(\bfx_{t-1} \mid \bfx_{t}, \bfx_{0})$, but with 
$\bfx_{0}$ expressed in terms of $\bfx_{t}$ and $\bm{\epsilon}_{\bftheta}(\bfx_{t},t)$
using Equation \ref{eq_fastforward}.



\subsubsection{DDIM}
Denoising Diffusion Implicit Models (DDIMs) \cite{song2020denoising} are designed to address the slow sampling speed of the original DDPMs \cite{ho2020denoising}. They can generate samples 10 to 50 times faster using a subset of sampling steps with minimal degradation in quality. In addition, DDIM can reuse pre-trained DDPM models for sampling acceleration without retraining.

The DDIM paper highlighted that many non-Markovian diffusion processes could have identical marginals (i.e., $q(\bfx_{t} \mid \bfx_{0})$) as DDPMs, and developed a more general reverse process (Figure \ref{fig:onestep} left):

\begin{equation}
\bfx_{t-1}=\sqrt{\bar{\alpha}_{t-1}}\cdot\underset{\text{predicted }\bfx_{0}\text{ from step } t} {\underbrace{\frac{\bfx_{t}-\sqrt{1-\bar{\alpha}_{t}}\bm{\epsilon}_{\bftheta}(\bfx_{t},t)}{\sqrt{\bar{\alpha}_{t}}}}}+\sqrt{1-\bar{\alpha}_{t-1}-\sigma_{t}^{2}}\cdot\bm{\epsilon}_{\bftheta}(\bfx_{t},t)+\sigma_{t}\mathbf{z}\label{eq_ddim_orig}
\end{equation}

\noindent where $\sigma_{t}=\eta\cdot\sqrt{(1-\bar{\alpha}_{t-1})/(1-\bar{\alpha}_{t})}\cdot\sqrt{\beta_{t}}$. Note that the generative process becomes a DDPM when setting $\eta$ to 1. 
%Our study employs a DDIM generative process by setting $\eta$ to 0 and uses a subset of time steps to expedite sampling (Section \ref{sec_method}).
Our method's reverse process is the same as the deterministic DDIM (i.e., $\eta = 0$), but with the deterministic noise $\bm{\epsilon}_{\bftheta}$
replaced by a random noise.

\subsection{Controllable Generation for MRI Reconstruction} % 
\label{sec:cg}


An uncontrolled generative process $p(\bfx)$ cannot be directly applied to MRI
reconstruction as it does not take the measurement $\bfy$ into account.
One possible generative approach for MRI reconstruction is to train a
conditional generative model $p(\bfx \mid \bfy)$.
However, this requires paired data and suffers from generalizability issues like
supervised methods.

A recent paper \cite{song2021solving} proposes a fully unsupervised generative
approach for solving inverse problems by first training an unconditional
diffusion model, and then guide the sampling process by using the known physics
model relating the image $\bfx$ and the measurement $\bfy$.
In MRI, the physics model is given by 
$\bfy=\mathbf{\Lambda}\mathbf{F}\bfx+\bm{\epsilon}$, where
$\mathbf{\Lambda}$ represents the binary k-space under-sampling mask, 
$\mathbf{F}$ denotes the forward Fourier transform, and 
$\bm{\epsilon}$ is the k-space measurement noise.
This is used to define a diffusion process in the measurement space:
$\bfy_{t} = \mathbf{\Lambda}\mathbf{F}\bfx_t+\alpha_{t} \epsilon$. 
At each reverse step, the prediction $\bfx_{t}$ is first computed from
$\bfx_{t+1}$ using the uncontrolled model, then a correction is applied as
follows:
a $\bfy_{t}$ value is sampled, and then $\bfx_{t}$ is corrected by projecting it
onto the hyperplane of 
$\{\bfx \mid \mathbf{\Lambda}\mathbf{F} \bfx = \bfy_{t}\}$ using the formula:
\begin{equation}
	\bfx_{t}
	\gets
	\mathbf{F}^{-1}[\mathbf{\Lambda}\bfy_{t}+(\bfI-\mathbf{\Lambda})\mathbf{F}\bfx_{t}] \label{eq_kspace}
\end{equation}
Sampling $\bfy_{t}$ can be done efficiently using the closed-form formula:
$\bfy_{t}=\sqrt{\bar{\alpha}_{t}}\cdot\bfy_{0}+\sqrt{1-\bar{\alpha}_{t}}\cdot\mathbf{\Lambda}\mathbf{F}\mathbf{z}$,
where $\mathbf{z}\sim \calN(\mathbf{0}, \bfI)$.

While this elegant technique allows fully unsupervised generative approach for
MRI reconstruction, it is computationally inefficient.
Our method extends this approach with a much more efficient high-fidelity
sampling strategy for the reverse process.
Our sampling strategy is inspired by DDIM, but note that direct DDIM acceleration can
lead to unsatisfactory reconstruction outcomes as the sampling trajectory can
fall outside the data manifolds.



\subsection{Method}
\label{sec_method}


Our Predictor-Projector-Noisor (PPN) method follows the fully unsupervised framework in \cite{song2021solving}.
Instead of using the measurement constrained reverse sampling process as 
described in Section \ref{sec:cg}, we provide a more efficient sampler that better exploit the measurement.

As shown in Figure \ref{fig:onestep}  and Equation \ref{eq_ddim_orig}, the unconditional DDIM involves a rough prediction of the noise-free sample $\mathbf{x}_0$ during each reverse step $\tau$. The PPN method adds an extra correction sub-step by projecting the estimated $\mathbf{x}_0$ onto the k-space measurement hyperplane of $\{\bfx \mid\mathbf{\Lambda}\mathbf{F}\bfx=\bfy\}$ before adding noise to return to a higher noise level $\bfx_{\tau-1}$, as shown in Figure \ref{fig_onestep}b. The reverse step of PPN from $\tau$ to $\tau-1$ can be formulated as:
\begin{equation}
\mathbf{x}_{\tau-1}=\sqrt{\bar{\alpha}_{\tau-1}}\cdot\text{Proj}\underset{\mathbf{x}_{0}^{(\tau)}:\text{ predicted }\mathbf{x}\text{ from step }\tau}{\underbrace{\left(\frac{\mathbf{x}_{\tau}-\sqrt{1-\bar{\alpha}_{\tau}}\bm{\epsilon}_{\bm{\theta}}(\mathbf{x}_{\tau},\tau)}{\sqrt{\bar{\alpha}_{\tau}}}\right)}}+\sqrt{1-\bar{\alpha}_{\tau-1}}\cdot\mathbf{z}\label{eq_ddim2}
\end{equation}
\noindent where $\mathbf{z} \sim \mathcal{N}(\bm{0},\bm{I})$, and

\begin{equation}
\text{Proj}(\bfx_{0}^{(\tau)})=\mathbf{F}^{-1}[\mathbf{\Lambda}\bfy+(\bfI-\mathbf{\Lambda})\mathbf{F}\bfx_{0}^{(\tau)}] \label{eq_kspace2}
\end{equation}
Unlike deterministic DDIM ($\eta = 0$), we replace $\bm{\epsilon}_{\bm{\theta}}(\mathbf{x}_{\tau},\tau)$ with $\mathbf{z}$, which has shown to improve our prediction performance according to our experimental results.

Our algorithm subtly transforms the unconditional DDIM to controllable generation by minimal changes, as seen in Algorithms \ref{alg:ppn}, which enables PPN to use DDIM for acceleration conveniently. For ease of notation, in Equations \ref{eq_ddim2} and \ref{eq_kspace2}, we use $\tau={0,\cdots, S}$ to denote the subset of the original time steps, and $S$ is substantially smaller than the original time steps $T$.  Note that our Equation \ref{eq_kspace2} is similar to Equation \ref{eq_kspace} proposed by \cite{song2021solving}. However, our projection is repeatedly performed only on the predicted $\mathbf{x}_0$ and measurement $\bfy$, instead of on $\mathbf{x}_t$ and $\mathbf{y}_t$, thereby eliminating $\mathbf{y}_t$. 

\input{sections/s2b.algorithm.tex}

==> sections/s3b.table3.tex <==
\begin{table}[t]
    \centering
    \caption{\FIX{Comparison}{fix here} of the running time of different algorithms for one single FFHQ 256x256 sample. All the methods are run with a single NVIDIA Tesla V100-PCIE GPU.}
    \vspace{5pt} % Adds 5 points of space between the caption and the table
    \begin{tabular}{c|c|c}
        \toprule
        \multirow{1}{*}{Method}  & \multicolumn{1}{c|}{Running time [s]} & \multicolumn{1}{c}{Memory [MB]} \\
        \midrule
        DDNM \cite{wang2022zero} &\pmvalue{0.675}{0.087} & \pmvalue{0.733}{0.060}  \\
        MedScore \cite{song2021solving}  & \pmvalue{0.719}{0.087} & \pmvalue{0.833}{0.049}    \\
        DPS \cite{chung2022dps}  & \pmvalue{0.709}{0.091} & \pmvalue{0.831}{0.071}  \\
        \midrule
        \rowcolor{lightgray}
        PPN (Ours) &\bpmvalue{0.827}{0.068} & \bpmvalue{0.918}{0.034}  \\
        \bottomrule
    \end{tabular} 
    \label{tab:result2}
\end{table}
